Towards Discriminative and Transferable One-Stage Few-Shot Object Detectors

Recent object detection models require large amounts of annotated data for training a new classes of objects. Few-shot object detection (FSOD) aims to address this problem by learning novel classes given only a few samples. While competitive results have been achieved using two-stage FSOD detectors, typically one-stage FSODs underperform compared to them. We make the observation that the large gap in performance between two-stage and one-stage FSODs are mainly due to their weak discriminability, which is explained by a small post-fusion receptive field and a small number of foreground samples in the loss function. To address these limitations, we propose the Few-shot RetinaNet (FSRN) that consists of: a multi-way support training strategy to augment the number of foreground samples for dense meta-detectors, an early multi-level feature fusion providing a wide receptive field that covers the whole anchor area and two augmentation techniques on query and source images to enhance transferability. Extensive experiments show that the proposed approach addresses the limitations and boosts both discriminability and transferability. FSRN is almost two times faster than two-stage FSODs while remaining competitive in accuracy, and it outperforms the state-of-the-art of one-stage meta-detectors and also some two-stage FSODs on the MS-COCO and PASCAL VOC benchmarks.

==> figures/qualitative.tex <==
\begin{figure*}[t!]
    \captionsetup[subfloat]{position=top, labelformat=empty, skip=0pt}
    \centering
    \begin{minipage}{0.95\textwidth}
    \subfloat[FSRN \hspace{2.5cm} Groundtruth]{\includegraphics[width=  0.49\textwidth, height=  0.333\textwidth]{qualitative/000000574823.jpg}} \hfill
    \subfloat[FSRN \hspace{2.5cm} Groundtruth]{\includegraphics[width=  0.49\textwidth, height=  0.333\textwidth]{qualitative/000000088485.jpg}}
    \par
    \vspace{-2em}
    \subfloat[]{\includegraphics[width=  0.49\textwidth, height=  0.333\textwidth]{qualitative/000000574315.jpg}} \hfill
    \subfloat[]{\includegraphics[width=  0.49\textwidth, height=  0.333\textwidth]{qualitative/000000575372.jpg}}
    \par
    \vspace{-2em}
    \subfloat[]{\includegraphics[width=  0.49\textwidth, height=  0.333\textwidth]{qualitative/000000575815.jpg}} \hfill
    \subfloat[]{\includegraphics[width=  0.49\textwidth, height=  0.333\textwidth]{qualitative/000000576052.jpg}}
    \par
    \vspace{-2em}
    \subfloat[]{\includegraphics[width=  0.49\textwidth, height=  0.333\textwidth]{qualitative/000000577149.jpg}} \hfill
    \subfloat[]{\includegraphics[width=  0.49\textwidth, height=  0.333\textwidth]{qualitative/000000581357.jpg}}
    \par
    \end{minipage}
    
   \caption{Qualitative results for the proposed FSRN model in 10-shot setting on MS-COCO dataset. }
   \label{fig:QUALITATIVE}
   %\vspace{-1em}
\end{figure*}


    


==> tables/ablation_anchors.tex <==
\begin{table}[t!]
\centering
\footnotesize
\setlength{\tabcolsep}{2.0 pt}
\caption[Effect of number of anchors]{\textbf{Effect of number of anchors.} Initially, Increasing the number of anchors leads to performance increase, however, it leads to training instability if learning capacity is not increased.}
\label{tab:anchors_effect}
\adjustbox{width=1.0\linewidth}{
\begin{tabular}{c|c|cccc|cccc}
\toprule
\multirow{2}{*}{\#Sizes} &  \multirow{2}{*}{\#Ratios}  & \multicolumn{4}{c|}{Base Performance} & \multicolumn{4}{c}{Novel Performance} \\ 
& &bAP  & bAP50     & bAP75    &  bAR   & nAP   & nAP50     & nAP75   & nAR  \\ \midrule
1 & 1  & 17.7 & 27.8 & 19.1 & 40.0 & 7.6 & 13.8 & 7.6 & 24.0 \\
3 & 3  & 27.5 & 40.5 & 29.8 & 46.6 & 13.0 & 22.0 & 13.0 & 29.6 \\
5 & 3  & \textbf{32.5} & \textbf{48.6} & \textbf{35.0} & \textbf{54.0} & {\bf 15.8} & {\bf 26.4} & {\bf 15.9} & {\bf 36.0}  \\
5 & 5  & \multicolumn{8}{c}{\multirow{2}{*}{no convergence (training instability)}}\\
7 & 7  & \multicolumn{8}{c}{} \\ 
\bottomrule
\end{tabular}}
\end{table}

==> tables/ablation_fl.tex <==
\begin{table}[h!]
\centering
\footnotesize
\setlength{\tabcolsep}{2.0 pt}
\caption[Effect of FL hyperparameters]{\textbf{Effect of FL hyperparameters.} We can see that our model is sensitive to the hyperparameters of the focal loss. This sensitivity is a problem faced by all meta-learners.}
\label{tab:fl_hyperparameters}
\adjustbox{width=1.0\linewidth}{
\begin{tabular}{cc|cccc|cccc}
\toprule
\multicolumn{2}{c|}{FL Parameters} & \multicolumn{4}{c|}{Base Performance} & \multicolumn{4}{c}{Novel Performance} \\  
$\gamma$ & $\alpha$ & bAP  & bAP50     & bAP75    &  bAR   & nAP   & nAP50     & nAP75   & nAR \\ \midrule
2 & 0.25 & \multicolumn{8}{c}{\multirow{2}{*}{no convergence (training instability)}} \\
2 & 0.5 & \multicolumn{8}{c}{} \\
4 & 0.25 & 24.3 & 38.0 & 26.4 & 40.6 & 12.6 & 23.0 & 12.3 & 30.8\\ 
4 & 0.5 & \textbf{32.5} & \textbf{48.6} & \textbf{35.0} & \textbf{54.0} & {\bf 15.8} & {\bf 26.4} & {\bf 15.9} & {\bf 36.0}  \\ 
\bottomrule
\end{tabular}}
\end{table}

==> tables/ablation_msda_mm.tex <==
\begin{table*}[t!]
	\addtolength{\tabcolsep}{3pt}
	\begin{center}
	\caption{{\bf Ablation study on MWST and MSDA.}
	We report the mean Averaged Precision and mean Averaged Recall on the 20 novel classes of MS-COCO in 10-shot setting.
	}
	\label{tab:ablation_msda}
    %\vspace{-2mm}
    \scalebox{1.0}{
	\begin{tabular}{c | c | c | cccc | cccc}
	\toprule
	\multirow{2}{*}{MWST} & \multirow{2}{*}{MSDA} & \multirow{2}{*}{$\mathcal{L}_{MM}$} & \multicolumn{4}{c}{Base Performance} & \multicolumn{4}{c}{Novel Performance} \\
	&  & & bAP & bAP50 & bAP75 & bAR & nAP & nAP50 & nAP75 & nAR \\
	\midrule
	\xmark&\cmark& \cmark & 23.7 &  34.5 &  25.7 &  45.4 & 13.0 & 22.3 & 13.1 & 28.4\\
	\cmark&\xmark& \xmark& 30.6 & 44.9 & 33.6 & 52.5 & 15.1 & 25.3 & 15.2 & 32.1\\
	\cmark&\cmark& \xmark& 30.6 & 44.9 & 33.6 & 52.5 & 15.4 & 25.7 & 15.9 & 33.1\\
	\cmark&\xmark & \cmark &30.6 & 44.9 & 33.6 & 52.5 & 15.4 & 26.4 & 15.8 & 34.1  \\
	\cmark&\cmark& \cmark& \textbf{32.5} & \textbf{48.6} & \textbf{35.0} & \textbf{54.0} & {\bf 15.8} & {\bf 26.4} & {\bf 15.9} & {\bf 36.0}  \\
	\bottomrule
	\end{tabular}}
	\end{center}
\end{table*}

==> tables/ablation_training.tex <==
\begin{table}[H]
	\addtolength{\tabcolsep}{4pt}
	\begin{center}
	\caption{{\bf Impact of MWST compared to contrasive training strategy.}
	We report the mean Averaged Precision and mean Averaged Recall on the 20 novel classes of MS-COCO in 10-shot setting.
	}
	\label{tab:ablation_mwst}
    %\vspace{-2mm}
    \scalebox{0.9}{
	\begin{tabular}{ c |cccc}
	\toprule
	\multirow{2}{*}{Method} & \multicolumn{4}{c}{Average Precision/Recall} \\
	& AP & AP50 & AP75 & AR \\
	\midrule
	Contrastive & 13.0 & 22.3 & 13.1 & 28.4\\
	MWST & {\bf 15.8} & {\bf 26.4} & {\bf 15.9} & {\bf 36.0}  \\
	\bottomrule
	\end{tabular} }
	\end{center}
\end{table}

